Ethical Considerations for Responsible Data Curation

Human-centric computer vision (HCCV) data curation practices often neglect privacy and bias concerns, leading to dataset retractions and unfair models. HCCV datasets constructed through nonconsensual web scraping lack crucial metadata for comprehensive fairness and robustness evaluations. Current remedies are post hoc, lack persuasive justification for adoption, or fail to provide proper contextualization for appropriate application. Our research focuses on proactive, domain-specific recommendations, covering purpose, privacy and consent, and diversity, for curating HCCV evaluation datasets, addressing privacy and bias concerns. We adopt an ante hoc reflective perspective, drawing from current practices, guidelines, dataset withdrawals, and audits, to inform our considerations and recommendations.

==> sections/summary_table.tex <==
\begin{table}[t]
    \caption{Summary of ethical considerations associated with current dataset collection practices and practical recommendations proposed to address these concerns.}
    % \Description{Summary of ethical considerations associated with current dataset collection practices and practical recommendations proposed to address these concerns.}
    \label{tab:summary}
    \centering
    \tiny
    \begin{tabular}{p{0.01\textwidth}p{0.43\textwidth}p{0.005\textwidth}p{0.43\textwidth}}
    \toprule
        & \textbf{Ethical considerations} & & \textbf{Practical recommendations}\\
    \midrule
         \raisebox{-2.5\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Purpose (Sec. \ref{purpose})}} & 
        \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
            \item Repurposing datasets for unintended uses 
            \item Fairness-unaware datasets are inadequate for measuring fairness
            \item Fairness-aware datasets are incompatible with common CV tasks
        \end{itemize}
        & & \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
            \item Refrain from repurposing existing dataset for fairness purposes
            \item Center dataset collection efforts on both the needs of the vision community and wider society
            \item Create a purpose statement prior to collecting data
        \end{itemize}\\
        \\
        \hdashline
        \raisebox{-6\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Consent and Privacy (Sec. \ref{consent_and_privacy})}} & 
         \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
            \item Collection efforts, such as the common paradigm of web-scraping, prioritize amassing data with unconstrained and uncontrolled practices 
            \item Collection efforts are not under the domain of existing research ethics institutions (e.g., Institutional Review Board)
            \item Dataset collectors have taken advantage of perceived ``loopholes'' in laws or licenses when in fact these actions can constitute illegal practice
            \item Data includes, or targets, vulnerable individuals
            \item Dataset collectors often neither obtain informed consent from image subjects nor provide a mechanism for consent withdrawal 
            \item Datasets often contain private information in the image or in the image metadata (e.g., geolocation, user-added comments)
        \end{itemize}
        &  &
        \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
          \item Obtain voluntary informed consent from all people depicted in, or identifiable from, a dataset
          \item Collect information on the country of residence to ensure that the dataset adheres to current and future laws
          \item Redact areas of the image that contain privacy-sensitive information (e.g., nonconsensual people, text)
          \item Redact metadata that contains privacy-sensitive information
        \end{itemize}\\
        \hdashline
        \raisebox{-7.5\normalbaselineskip}[0pt][0pt]{\rotatebox[origin=c]{90}{Diversity (Sec. \ref{diversity})}} & \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
            \item Human-centric datasets reflect historical and representational biases which can also lead to disparate algorithmic performance
            \item Populations with no or less access to digital technology lack sufficient representation in datasets
            \item Taxonomies used to label demographics can reify harmful social structures 
            \item Own-anchor bias and reliance on nonphysiological markers to infer physiological markers
            \item Erasure of nonstereotypical individuals 
            \item Incorrect perception that demographic labels fully describe the axes of human variability
            \item Factors related to the instrument (e.g., camera) and environment are overlooked as causes for model performance differences
            \item Data annotators introduce their own biases but little to no information is provided about them
            \item Data annotators face exploitative and uncertain work conditions
        \end{itemize}
        & &
        \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
        \item Obtain self-reported annotations rather than relying on inference
        \item Provide open-ended responses options
        \item Acknowledge the multiplicity of identity by allowing individuals to select multiple options for identity categories
        \item Acknowledge the mutability of identity and ask for self-identified information at time of image capture
        \item Collect aggregate data for commonly ignored sensitive attributes 
        \item If collecting the following annotations, we recommend the following schema:
            \begin{itemize}[leftmargin=1cm,topsep=0pt,itemsep=-2pt]
              \item Exact biological age at time of image capture
              \item Self-identified pronouns at time of image capture
              \item Ancestry rather than ethnicity or race
            \end{itemize}
        \item We also recommend collecting the following annotations: phenotypic attributes (e.g., hair type), environment information, and instrument data
        \item Recontextualize annotators as contributing factors
        \item Compensate annotators and data subjects fairly (i.e., above their country's minimum wage and according to the complexity of the task)
        \end{itemize}
        \\
    \bottomrule
    \end{tabular}
\end{table}


% \begin{table}[t]
%     \caption{Summary of ethical considerations associated with current dataset collection practices and practical recommendations proposed to address these concerns.}
%     % \Description{Summary of ethical considerations associated with current dataset collection practices and practical recommendations proposed to address these concerns.}
%     \label{tab:summary}
%     \centering
%     \tiny
%     \begin{tabular}{p{0.45\textwidth}p{0.01\textwidth}p{0.45\textwidth}}
%     \toprule
%         \textbf{Ethical considerations} & & \textbf{Practical recommendations}\\
%     \midrule
%         \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
%             \item Repurposing datasets for unintended uses 
%             \item Fairness-unaware datasets are inadequate for measuring fairness
%             \item Fairness-aware datasets are incompatible with common CV tasks
%         \end{itemize}
%         & & \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
%             \item Refrain from repurposing existing dataset for fairness purposes
%             \item Center dataset collection efforts on the needs of the vision community and wider society
%             \item Create a purpose statement prior to collecting data
%         \end{itemize}\\
%         \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
%             \item Collection efforts prioritize amassing data with uncontrolled practices 
%             \item Dataset collectors have taken advantage of legal ``loopholes'' when in fact these actions can constitute illegal practice
%             \item Data includes, or targets, vulnerable individuals
%             \item Dataset collectors often neither obtain informed consent from image subjects nor provide a mechanism for consent withdrawal 
%             \item Datasets often contain private information in the image or in the image metadata (e.g., geolocation, user-added comments)
%         \end{itemize}
%         &  &
%         \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
%           \item Obtain voluntary informed consent from all people depicted in a dataset
%           \item Collect information on the country of residence to ensure that the dataset adheres to current and future laws
%           \item Redact areas of the image that contain privacy-sensitive information and sensitive metadata
%         \end{itemize}\\
%         \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
%             \item Human-centric datasets reflect historical and representational biases
%             \item Populations with no or less access to digital technology lack sufficient representation in datasets
%             \item Own-anchor bias and reliance on nonphysiological markers to infer physiological markers
%             \item Erasure of nonstereotypical individuals 
%             \item Incorrect perception that demographic labels fully describe the axes of human variability
%             \item Factors related to the instrument (e.g., camera) and environment are overlooked as causes for model performance differences
%             \item Data annotators introduce their own biases but little to no information is provided about them
%             \item Data annotators face exploitative and uncertain work conditions
%         \end{itemize}
%         & &
%         \begin{itemize}[leftmargin=0cm,topsep=0pt,itemsep=-2pt]
%         \item Obtain self-reported annotations rather than relying on inference
%         \item Provide open-ended responses options
%         \item Acknowledge the multiplicity of identity by allowing individuals to select multiple options for identity categories
%         \item Acknowledge the mutability of identity and ask for self-identified information at time of image capture
%         \item Collect aggregate data for commonly ignored sensitive attributes 
%         \item If collecting the following annotations, we recommend the following schema:
%             \begin{itemize}[leftmargin=1cm,topsep=0pt,itemsep=-2pt]
%               \item Exact biological age at time of image capture
%               \item Self-identified pronouns at time of image capture
%               \item Ancestry rather than ethnicity or race
%             \end{itemize}
%         \item We also recommend collecting the following annotations: phenotypic attributes (e.g., hair type), environment information, and instrument data
%         \item Recontextualize annotators as contributing factors
%         \item Compensate annotators and data subjects fairly (i.e., above their country's minimum wage and according to the complexity of the task)
%         \end{itemize}
%         \\
%     \bottomrule
%     \end{tabular}
% \end{table}

            % \item Derivative datasets can repurpose existing datasets for unintended use cases 
            % \item Datasets created without fairness explicitly in mind will be inadqueate for mitigating or studying algorithmic bias
            % \item Existing fairness-aware datasets are incompatible with common computer vision tasks (e.g., dataset size, task narrowness) 
